Analysis of Optical Loss and Crosstalk Noise in MZI-based Coherent Photonic Neural Networks

With the continuous increase in the size and complexity of machine learning models, the need for specialized hardware to efficiently run such models is rapidly growing. To address such a need, silicon-photonic-based neural network (SP-NN) accelerators have recently emerged as a promising alternative to electronic accelerators due to their lower latency and higher energy efficiency. Not only can SP-NNs alleviate the fan-in and fan-out problem with linear algebra processors, their operational bandwidth can match that of the photodetection rate (typically 100 GHz), which is at least over an order of magnitude faster than electronic counterparts that are restricted to a clock rate of a few GHz. Unfortunately, the underlying silicon photonic devices in SP-NNs suffer from inherent optical losses and crosstalk noise originating from fabrication imperfections and undesired optical couplings, the impact of which accumulates as the network scales up. Consequently, the inferencing accuracy in an SP-NN can be affected by such inefficiencies -- e.g., can drop to below 10% -- the impact of which is yet to be fully studied. In this paper, we comprehensively model the optical loss and crosstalk noise using a bottom-up approach, from the device to the system level, in coherent SP-NNs built using Mach-Zehnder interferometer (MZI) devices. The proposed models can be applied to any SP-NN architecture with different configurations to analyze the effect of loss and crosstalk. Such an analysis is important where there are inferencing accuracy and scalability requirements to meet when designing an SP-NN. Using the proposed analytical framework, we show a high power penalty and a catastrophic inferencing accuracy drop of up to 84% for SP-NNs of different scales with three known MZI mesh configurations (i.e., Reck, Clements, and Diamond) due to accumulated optical loss and crosstalk noise.

==> static_power_texts.tex <==
\subsection{Power Analysis of MZI-based SiPh Accelerators}\label{power_analysis_model}
The static power consumption in SP-NNs is dominated by the tuning power required to achieve specific phase settings for $\theta$ and $\phi$ in each MZI in the OIUs. Considering implementing the phase shifters using microheaters, this power consumption in SP-NNs depends on the microheater's geometry such as its width, thickness, distance with the waveguide, and length as well as the number of the MZIs in the OIUs, and the required phase settings. In this paper, the heater material considered is Ti/TiN with $\rho=$~60~$\mu\Omega$.cm and sheet resistance of 5.5~$\Omega$/sq. The thickness of the heater is 110~nm with a width and length of 0.42~$\mu$m and 40~$\mu$m, respectively, placed 150~nm above the waveguide \cite{shafiee2023design}.

To perform static power analysis, we designed a microheater-based phase shifter for MZIs based on strip waveguides and considering the central frequency of 1550 nm. The multiphysics utility of Synopsys Rsoft CAD \cite{RsoftCAD} was used to carry out the performance analysis of the phase shifter.
%of a single phase shifter with a similar design to \cite{Farhad_4by4} but for a central frequency of 1550 nm. 
The simulation results showing the achieved phase shift as a function of the applied voltage to the microheater are shown in Fig.~\ref{Fig:: PS}. Note that the width of the strip waveguide is considered to be 420~nm to ensure single-mode propagation of the optical signal.
%As it was mentioned before, MZIs in OIUs and optoelectronic NAUs may take more than two intermediate states. 
 To analyze the static power consumption of the entire SP-NN, having an analytical model to analyze the bias voltage as a function of the phase settings and vice versa is critical. To do so, we fit a second-order polynomial with an R2 score of 0.99 to the simulation results from Rsoft CAD, shown in Fig.~\ref{Fig:: PS}. 
\begin{figure}[t]
\centering
\includegraphics[width=3.5in]{figures_TVLSI/PS_final.pdf}
  \caption{Phase shifter's phase as a function of the applied voltage to a microheater used in a 2$\times$2 MZI multiplier.}\label{Fig:: PS}
  \vspace{-0.15in}
\end{figure}

Utilizing the defined analytical models and taking into account $R\approx 507$ $\Omega$ of resistance of each microheater \cite{Farhad_4by4}, we can calculate the total static power consumption in any SP-NN with an arbitrary architecture by having the trained phase settings of $\phi$ and $\theta$ and using Ohm's law, as shown below ($\Theta=\theta$ or $\phi$):

\begin{equation*}
    P_{stat}(\Theta)=\frac{V(\Theta)^2}{R}. \tag{12} \label{Eq::static_power}
\end{equation*}
%($P_{stat}(\theta)=\frac{V(\theta)^2}{R}$ and $P_{stat}(\phi)=\frac{V(\phi)^2}{R}$).










\subsection{Phase Shifter's Power Consumption}
 To maintain the phase settings $\theta$ and $\phi$ on each MZI in SP-NNs' OIUs, a bias voltage must be applied to each phase shifter. Depending on the required phase settings per MZI, the required bias voltage changes, and hence the total static power consumption per MZI and the entire SP-NN change. To calculate the total static power consumption in SP-NNs, we extend the analytical model defined in \ref{power_analysis_model} for each phase shifter to the full network with 1000 pairs of $\theta$ and $\phi$ using a normal distribution with (mean) $\mu=\pi/2$ and (standard deviation) $\sigma=\pi/2$ for $\theta$ and $\mu=\pi$ and $\sigma=\pi$ for $\phi$. 

As it can be seen from Fig. \ref{Fig:: static_power}, with an increase in the number of input ports and network layers ($M$), the static power consumption due to the bias voltage of the phase shifter increases. Such an increase in the static power consumption is due to the increase in the number of MZIs required in SP-NNs, and hence phase shifters when scaling the network. We can see from Fig. \ref{Fig:: static_power} that the average and worst-case static power consumption for a single 8$\times$8 ($M=$~1 and $N=$~8) with Clements or Reck mesh can be as low as 4.51~W and 6.6~W, respectively. Moreover, the average and worst-case static power consumption can be as high as 382.2~W and 412.84~W, respectively, for 3 layers with 64 inputs ($M=$~3 and $N=$~64). As for the Diamond configuration, because of a higher number of MZIs in the mesh structure, for a single-layer SP-NN network with 8 inputs, the average power consumption is 6.25~W. As we scale the Diamond network, the average and worst-case static power consumption increases drastically and can be as high as 750~W and 819.4~W, respectively for 3 layers of SP-NNs with 64 inputs. Note that in all of these simulations, the SOA power consumption (540 mW per unit) and optoelectronic NAU power consumption are not considered in the total static power consumption. 
\begin{figure}[t]
\centering
\includegraphics[width=3.6 in]{figures_TVLSI/static_box_final.pdf}
  \caption{ Static power consumption analysis of SP-NNs for different mesh configurations and scales. }\label{Fig:: static_power}
  \vspace{-0.2in}
\end{figure}
While the results in Fig.~\ref{Fig:: static_power} show similar static power consumption for Reck and Clements configuration, for the same weight matrix, their static power consumption might not be the same. The reason for this is that the same weight matrix will be decomposed differently in the two mesh configurations, hence leading to different phase settings. For example, for the case where we have an SP-NN with 2 hidden layers ($M=$~3) and 16 inputs trained on the FFT-MNIST dataset, the network's static power consumption is 24~W when using Clements, 27.22~W when using Reck, and 38.27~W when Diamond mesh is used.

 It was demonstrated in \cite{mirza2022characterization} that increasing the width of the waveguide could increase the resilience of the network to fabrication-process imperfections. Nevertheless, our multiphysics simulation for microheaters shows that as we increase the width of a waveguide, the required voltage to impose a $\pi$ phase shift on the underlying waveguide also increases. In addition, the metallic loss also increases due to the increased area of the metal contacts.
 %Consequently, leveraging the method proposed in \cite{mirza2022characterization} would come at a cost of up to two-fold increased static power consumption of SP-NNs. 
 The proposed analysis for static power consumption helps SiPh designers to better explore the scale and configuration for the SP-NN based on the application-dependent power consumption budget. In addition, the proposed analyses motivate the need for designing phase shifters with lower static power consumption to maintain the phase shift values in the SP-NNs.

